Composition of Experts: A Modular Compound AI System Leveraging Large Language Models

Large Language Models (LLMs) have achieved remarkable advancements, but their monolithic nature presents challenges in terms of scalability, cost, and customization. This paper introduces the Composition of Experts (CoE), a modular compound AI system leveraging multiple expert LLMs. CoE leverages a router to dynamically select the most appropriate expert for a given input, enabling efficient utilization of resources and improved performance. We formulate the general problem of training a CoE and discuss inherent complexities associated with it. We propose a two-step routing approach to address these complexities that first uses a router to classify the input into distinct categories followed by a category-to-expert mapping to obtain desired experts. CoE offers a flexible and cost-effective solution to build compound AI systems. Our empirical evaluation demonstrates the effectiveness of CoE in achieving superior performance with reduced computational overhead. Given that CoE comprises of many expert LLMs it has unique system requirements for cost-effective serving. We present an efficient implementation of CoE leveraging SambaNova SN40L RDUs unique three-tiered memory architecture. CoEs obtained using open weight LLMs Qwen/Qwen2-7B-Instruct, google/gemma-2-9b-it, google/gemma-2-27b-it, meta-llama/Llama-3.1-70B-Instruct and Qwen/Qwen2-72B-Instruct achieve a score of $59.4$ with merely $31$ billion average active parameters on Arena-Hard and a score of $9.06$ with $54$ billion average active parameters on MT-Bench.

==> CoE_Experiments.tex <==
\section{Experimental Setup}\label{sec:experimental_setup}
We evaluate the two-step routing based CoEs. 

We evaluate the CoE approach for the expert set $\mathcal{E}$  comprising of the following well known open weight LLMs: 
\textit{Qwen/Qwen2-7B-Instruct, google/gemma-2-9b-it, google/gemma-2-27b-it, meta-llama/Llama-3.1-70B-Instruct and Qwen/Qwen2-72B-Instruct}.

We consider the following domain categories: Medical, Finance, Coding/Computer Programming, Mathematics, and Law; and the following languages categories: Arabic, Serbian, Slovenian, Hungarian, Russian, Turkish, Japanese and Thai. We source high quality seed prompts for these domain categories with domain specific open-source datasets available on HuggingFace. We restrict only to the training splits to avoid contamination with benchmarks. The dataset used for each domain is listed in Table \ref{tab:domain_dataset_sources} in the Appendix. We construct multilingual prompts in various formats such as native, translation, and cross-lingual for all the language categories. The exact methodology and source datasets are outlined in Section \ref{sec:multilingual_category} in the Appendix. 

Equipped with these high quality category labeled seed prompts extend prompt dataset by following the semi-supervised pipeline in Figure \ref{fig:training_data_pipeline} on general chat prompts from internal user trials and training split \cite{lmsys-chatbot-arena}. We use \textit{intfloat/e5-mistral-7b-instruct} as the text embedding model given its strong performance on Massive Multitask Embedding Benchmark \cite{muennighoff2023mtebmassivetextembedding} and train $k$-NN classifier on seed prompt set. We measure confidence in terms of entropy obtained by probabilities that the classifier assigns to various categories and we filter out prompts with entropy greater than $0.5$. In this manner, curated about $58000$ high quality category labeled prompts.  
\begin{figure}        
\centering
    \includegraphics[width=0.625\linewidth]{figs/pie_chart_router_training_data.png}
    \caption{Prompt category distribution in the router training data.}
    \label{fig:router_cat_distribution}
\end{figure}
The Figure \ref{fig:router_cat_distribution} shows category distribution for the final training data. %For each category we collected as many examples as possible to cover a wider variety of natural prompts in various categories. 

% In Figure \ref{fig:2d_tsne_plot_category}, we show that the router 2D t-SNE plot obtained via a powerful text embedding model \emph{intfloat/e5-mistral-7b-instruct} and colors indicate label indicating category of each prompt. We observe that prompts tend to cluster naturally into different categories indicating  that these embeddings informative enough for for building an accurate category router.
%Since the category-router $\textrm{CR}(\cdot)$ is a mapping from text to categories, we chose its architecture to comprising of a $k$-NN classifier built on top of a text-to-embedding backbone. 

Figure \ref{fig:2d_tsne_plot_category} shows the 2D t-SNE plot of prompt embeddings obtained from text-embedding model \textit{intfloat/e5-mistral-7b-instruct} and with colors indicating the category label of each prompt. The clustering of different categories into distinct cluster shows that these embeddings from  \textit{intfloat/e5-mistral-7b-instruct} are informative enough for building a highly accurate category router. 

\begin{figure}
     \centering
     \includegraphics[width=0.90\linewidth]{figs/prompt_2d_tsne_cat.png}
     \caption{2D t-SNE plot for prompts in the CoE training data with labels based on various categories comprising of variety of domains and languages.
    }
    \label{fig:2d_tsne_plot_category}
\end{figure} 

Encouraged by this, we choose category router $\textrm{CR}(\cdot)$  architecture as the $k$-NN classifier built on top of a text-to-embedding backbone. We train the category router on top of \textit{intfloat/e5-mistral-7b-instruct} embeddings and use a simple $k$-NN multi-class classifier.
We split the given training data into train, test and validation splits. We train $k$-NN for various of $k=10, 15, 20, 25, 30, 35, 40$. The router accuracy on training and validation split for various values of $k$ is shown in Figure \ref{fig:train_val_error_plot}. Based on accuracy in validation split we choose $k=30$ for $k$-NN. The router achieves $98\%$ accuracy on the test and the confusion matrix is shown in the Figure \ref{fig:confusion_matrix}. It is quite evident from the confusion matrix that very high accuracy for category router can be achieved.

For the Robust-CoE, we choose entropy obtained from the probabilities that the $k$-NN classifier assigns to various categories. If the measured entropy for a given prompt is larger than the entropy threshold $\epsilon_{t}$ we assign it to 'general' category. We consider various values of $\epsilon_{t} \in \{0.05, 0.10, \cdots, 1.5 \}$ we choose the entropy threshold that leads minimal reduction in the recall of the trained category-router. 
\begin{figure}
     \centering
    \includegraphics[scale=0.50]{figs/cat_router_train_val_loss.png}
    \caption{Training validation accuracy vs. $k$ for $k$-NN based category router $\textrm{CR}$ using \textit{intfloat/e5-mistral-7b-instruct} as the text embedding model.}
    \label{fig:train_val_error_plot} 
\end{figure}
\begin{figure}
     \centering
    \includegraphics[scale=0.50]{figs/confusion_matrix.png}
    \caption{Confusion matrix on the test split for $k$-NN ($k=30$) based the category router $\textrm{CR}$ using \textit{intfloat/e5-mistral-7b-instruct} as the text embedding model.}
    \label{fig:confusion_matrix} 
\end{figure}
Based on this, we choose $\epsilon_{t} = 0.1$ for the Robust-CoE.  

For solving the category-to-expert mapping a desired completion for each prompt is required. We choose this completion as the response from the \emph{GPT-4o-2024-02-15-preview} with goal of constructing a CoE to match the quality of large state-of-art model. 

We obtain, $l_{i,j}$ in category-to-expert mapping optimization problem \eqref{eqn:MILP_Complicated} by computing the win-rate of $j^{th}$ expert on set of prompts routed to category $i^{th}$ using LLM-as-a-judge and equating $l_{i,j}$ as the negative of the win-rate. We use the judge prompt template in \cite{raju2024constructing} given its emphasis on effectively addresses the nuances associated with using LLM as a judge for variety of domains. We use \emph{GPT-4o-mini} as the judge model and generate judgment for expert completion in terms of whether it is similar or better and worse than the desired completion. Equipped with these judgments calculate win-rate expert $j$ on category $i$.  %This overall workflow is shown in Figure \ref{fig:Winrate_Computation}.

Equipped with $l_{i,j}$, we solve \eqref{eq: MILP} to obtain category-to-expert mapping for various values of parameter budget $B
\in \{7, 16, 35, 105, 190\}$ in billions of parameters. 

Figure \ref{fig:CoE_Test_Set_Performance} shows performance of CoEs and Robust CoEs for various values of $B$. We observe that the winrates for CoEs w.r.t \emph{GPT-4o-2024-02-15-preview} improves as we increase $B$ and they perform better individual experts. This shows performance w.r.t. large monolithic models can be improved via using CoE constructed out of readily available open source/weight models. We also observe that the performance of both CoE and Robust CoE are similar. This similarity in performance can be attributed to the fact that category-to-expert mapping chooses the best expert for the prompts routed to the `general' category and presence of strong general models in the expert pool. 

\begin{figure}
    \centering
    \includegraphics[scale=0.52]{figs/winrate_for_CoE.png}
    \caption{Win-rates against large monolithic model GPT-4o-2024-02-15-preview on on the test split vs. $B$ for experts LLMs, CoE and Robust-CoE. Various CoEs use $k$-NN ($k=30$) based category router using \textit{intfloat/e5-mistral-7b-instruct} as the text embedding model and category-to-expert mapping with parameter budget $B$.}
    \label{fig:CoE_Test_Set_Performance} 
\end{figure}



% \begin{figure*}
%     \centering
%     \includegraphics[width=1\linewidth]{figs/Category_to_Expert_Winrate.png}
%     \caption{Winrate Computation}
%     \label{fig:Winrate_Computation}
% \end{figure*}

\section{Experimental Results}
% \begin{figure*}[ht]
% \begin{minipage}[b]{0.33\textwidth}
%      \centering
%     \includegraphics[scale=0.3]{figs/cat_router_train_val_loss.png}
%     \caption{Training validation accuracy vs. $k$}
%     \label{fig:train_val_error_plot} 
% \end{minipage}
% \begin{minipage}[b]{0.33\textwidth}
%      \centering
%     \includegraphics[scale=0.3]{figs/confusion_matrix.png}
%     \caption{Confusion matrix on test data.}
%     \label{fig:confusion_matrix}    
% \end{minipage}
% \begin{minipage}[b]{0.33\textwidth}
%     \centering
%     \includegraphics[scale=0.3]{figs/winrate_for_CoE.png}
%     \caption{CoE winrates on test split.}
%     \label{fig:CoE_Test_Set_Performance}  
% \end{minipage}
% \end{figure*}

We evaluate the CoEs for different values of $B \in \{7, 16, 35, 105, 190\}$  on popular LLM Benchmarks such as Arena-Hard \cite{Arena_Hard}, MT-Bench \cite{MT_Bench} and various domain knowledge specific benchmark in MMLU-Pro \cite{MMLU_Pro}. We choose Arena-hard for measuring single-turn evaluations and MT-Bench to measure multi-turn evaluations for CoEs. These benchmarks contain challenging prompts collected in a crowd-sourced manner via Chatbot-Arena and represent a real-world usage of LLMs \cite{chiang2024chatbotarenaopenplatform}. For all the benchmark we measure performance against average number of active parameters for that benchmark. This can be obtained by taking average of the size of the expert chosen by the router for prompts in the benchmark.  We emphasize on measuring average number of parameters because it translates to better tokens per second and time-to-first-token. These some of the key metrics in real-world LLM applications.  

\subsection{Arena-Hard}

\begin{figure}
    \centering
        \includegraphics[scale=0.5]{figs/arena_hard.png}
        \caption{Area-Hard scores vs. average number of active parameters in Billions for expert LLMs, CoEs and Robust-CoEs.}
        \label{fig:arena-hard}
\end{figure}



% \begin{figure*}[htb]
%     \centering
%     \begin{minipage}[b]{0.33\textwidth}
%         \includegraphics[scale=0.35]{figs/arena_hard.png}
%         \caption{Arena-Hard}
%         \label{fig:arena-hard}
%     \end{minipage}
%     \begin{minipage}[b]{0.33\textwidth}
%         \includegraphics[scale=0.35]{figs/MT_Bench_Average.png}
%         \caption{MT-Bench} \label{fig:MT_Bench_Average}
%         \label{fig:MT_Bench_Results}
%     \end{minipage}
%     \begin{minipage}[b]{0.33\textwidth}
%         \centering
%         \includegraphics[scale=0.35]{figs/knowledge_intensive.png}
%         \caption{Knowledge Intensive Benchmarks}
%         \label{fig:Knowledge Intensive}
%     \end{minipage}    
% \end{figure*}

Figure \ref{fig:arena-hard} shows performance on the Arena-Hard benchmark for CoE for various values of $B$. On the y-axis is the the Arena-Hard score and on the $x$-axis is the average number of active parameters for the benchmark. As total size $B$ of CoE increases, CoE achieves better performance with fewer active performance and is better than individual experts. This shows that the performance of CoE scales as more experts added. We also observe that Robust-CoE significantly outperforms CoE, demonstrating the value of uncertainty quantified routing. It is key to the stable performance of CoE beyond the training dataset. The CoE and Robust-CoE with total parameters $B=190$ Billion achieves the score $60.2$ and $62.10$ with merely $65.23$ and $69.81$ Billion active parameters. Some of popular closed sourced model \emph{claude-3-opus-20240229}, \emph{gemini-1.5-flash-api-preview} and \emph{gpt-4-0613} achieve scores $60.4, 49.6$ and $37.9$ respectively. Due to closed sourced nature of these models, the number of parameters are not known. While the CoE is not state-of-art models on the benchmark, the performance of CoEs can be improved by easily by including new models that being actively developed by community leveraging the modular architecture of CoE.

\subsection{MT-Bench}
The performance on various metrics on MT-Bench and the average number of active parameters in the CoE are shown in Figure \ref{fig:MT_Bench_Results}. This benchmark measures performance of LLMs on multi-turn conversation. The CoE routes based on current input and then passes the entire conversation history. This means different experts might be chosen for different conversation turns. Figure \ref{fig:MT_Bench_Average} shows the average score over multi-turn conversations in the benchmark and average number of active parameters. They achieve similar performance to large expert models \emph{meta-llama/Llama-3.1-70B-Instruct} and \emph{Qwen/Qwen2-72B-Instruct}  at a much reduced average active parameters. 

\begin{figure}
    \centering
        \includegraphics[scale=0.5]{figs/MT_Bench_Average.png}
        \caption{Average MT-Bench scores vs. average number of active parameters in Billions for expert LLMs, CoEs and Robust-CoEs.} \label{fig:MT_Bench_Average}
        \label{fig:MT_Bench_Results}
\end{figure}



\subsection{Knowledge Intensive Benchmarks}
We measure the performance of CoE on knowledge intensive benchmarks such GSM8k CoT and MMLU-pro benchmark on the following subjects:  Mathematics, Business, Computer Science, Economics, Health and Law. The average score on these benchmarks vs. average number of active parameters are shown in Figure \ref{fig:Knowledge Intensive}.  We observe that while CoE does suffer from reduced performance as compared to individual experts, the Robust-CoE recovers most of this performance.  The fine-grained results are shown in Table \ref{tab:kt_benchmark_results}.  This can be attributed to the fact that the distribution mismatch between knowledge intensive tasks and the router training data. The robust-CoE via uncertainty quantification detects this mismatch and appropriately routes these prompts to the best generalist expert.

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figs/knowledge_intensive.png}
    \caption{Average scores on knowledge intensive benchmarks vs. average number of active parameters in Billions for expert LLMs, CoEs and Robust-CoEs.}
    \label{fig:Knowledge Intensive}
\end{figure}

\begin{table*}
    \centering
    \tiny
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
    \hline
       Model & GSM8k CoT & MMLU Pro   &  MMLU Pro   & MMLU Pro  & MMLU Pro  &  MMLU Pro  & MMLU Pro &  MMLU Pro & Average   \\
         & (Flexible Match) & Biology  &  Business  & Computer Science   &  Economics  &   Health & Law &  Math &  Score \\
    \hline
       Qwen2-7B-Instruct  &   0.780 & 	0.648 &	0.512 &	0.448 &	0.581 &	0.465 &	0.299	& 0.419	& 0.519\\
    \hline
        gemma-2-9b-it  &	0.816	& 0.768	& 0.523	& 0.487& 	0.643	& 0.592 &	0.346 &	0.441	& 0.577 \\
    \hline
        gemma-2-27b-it   &	0.844 &	0.785&	0.556	&0.597&	0.699	& 0.647&	0.415&	0.507&	0.631 \\
    \hline
       Llama-3.1-70B-Instruct 	& 0.924 &	0.779 &	0.618 &	0.629 &	0.738&	0.657 &	0.458 &	0.547 &	0.669\\
    \hline
        Qwen2-72B-Instruct  & 0.901 &	0.813 &	0.637	 & 0.639 & 0.763	& 0.667	 & 0.423	& 0.620 &	0.683\\
    \hline
       CoE 7B & 0.780 & 0.648 & 0.512 & 0.448 & 0.581 & 0.465 & 0.299 & 0.419 & 0.519 \\
       \hline
       CoE 16B & 0.780	 & 0.695 &	0.522 &	0.463	&0.643&	0.459&	0.344&	0.419&	0.541 \\
       \hline
       CoE 35B &  0.844 & 0.739 &	0.448 &	0.568&	0.522&	0.505	&0.415&	0.507	&0.569 \\
       \hline
       CoE 105B &  0.780 &	0.726 & 0.556&	0.514&	0.700&	0.664	&0.415&	0.419	&0.597 \\
       \hline
       CoE 190B & 0.901 &	0.781 & 0.447&	0.604	&0.523	&0.664	&0.415	&0.620	&0.619 \\
       \hline
      Robust CoE 7B & 0.780 & 0.648 & 0.512 & 0.448 & 0.581 & 0.465 & 0.299 & 0.419 & 0.519  \\
       \hline
      Robust CoE 16B & 0.780 &	0.767 &	0.523 &	0.487 &	0.643 &	0.577 &	0.344 &	0.423 &	0.568 \\
       \hline
      Robust CoE 35B & 0.844 &	0.785 &	0.556 &	0.597 &	0.699 &	0.624 &	0.415 &	0.507 &	0.628\\
       \hline
      Robust CoE 105B & 0.844 & 0.785	 & 0.556 &	0.597 &	0.699 &	0.637 &	0.415 &	0.507 &	0.630 \\
       \hline
      Robust CoE 190B & 0.901	& 0.781	& 0.618	& 0.626 &	0.738 &	0.664 &	0.422 &	0.620 &	0.671 \\
       \hline    
    \end{tabular}
    \newline
    \caption{\small Performance on knowledge intensive domain specific benchmarks.}
    \label{tab:kt_benchmark_results}
\end{table*}
